F-StrIPE: Fast Structure-Informed Positional Encoding for Symbolic Music Generation

While music remains a challenging domain for generative models like Transformers, recent progress has been made by exploiting suitable musically-informed priors. One technique to leverage information about musical structure in Transformers is inserting such knowledge into the positional encoding (PE) module. However, Transformers carry a quadratic cost in sequence length. In this paper, we propose F-StrIPE, a structure-informed PE scheme that works in linear complexity. Using existing kernel approximation techniques based on random features, we show that F-StrIPE is a generalization of Stochastic Positional Encoding (SPE). We illustrate the empirical merits of F-StrIPE using melody harmonization for symbolic music.

==> IEEEbib/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> sections/entropy.tex <==
At half-beat resolution

1024     0.03729058455519981 +- 0.008084586791244268
        Max:  0.06346470255685625       Min:  0.005513509114583333
4096     0.019980952965336557 +- 0.0037712786910756115
        Max:  0.027578312279776283      Min:  0.009592692057291666

==> sections/methods.tex <==
\section{Methods} \label{section:methods}

\subsection{Structure-informed Positional Encoding}

As we hinted in Section \ref{section:background}, positional encoding depends on a sequence $\mathcal{P} = [ p_1, p_2, ... , p_T ]$ of positional indices. In standard PE, which does not utilize structure, $p_i = i$, which makes $\mathcal{P}$ a linear grid. When structure is included in PE, $p_i = s_\ell (i)$, where $s_\ell (i)$ gives the structural label at level $\ell$ (e.g. chord) for timestep $i$. In this case, $s_\ell (i) = s_\ell (i^{\prime})$ is possible for $i \neq i^{\prime}$, making $\mathcal{P}$ a non-linear grid. In fact, we can consider vectorial positional indices with multiple resolutions of structural organization. Consequently, we obtain $p_i = \mathbf{s} (i)$, where $\mathbf{s} (i) = [ s_1 (i) , ..., s_\ell (i), ..., s_L (i) ]$ is a vector of $L$ structural labels. Viewed in this way, PEs with structure can simply be used as a drop-in replacement for PEs without structure by replacing the form of $p_i$, giving us richer positional information. This is a way to flexibly represent domain-specific prior knowledge about the underlying data domain.

\subsection{Asymptotic case of SPE: Random Fourier Features} \label{ssection:asymptotic_rff}

We can express the SFF approximation of the positional matrix $\mathbf{P}_d$ for arbitrary timesteps $m$ and $n$ as:
\begin{equation} \label{eq:sff_mn}
    \mathbf{P}_d[m, n] \approx \left[ \Omega_\mathcal{Q}^d [m, :] (\mathbf{Z}_d \mathbf{Z}_d^\top) \Omega_\mathcal{K}^{d^\top} [:, n] \right] / R \\
\end{equation}

where we use the abbreviation $\Omega_\mathcal{A}^d = \boldsymbol{\Omega}\left(\mathcal{P}_\mathcal{A}, \boldsymbol{f}_d, \boldsymbol{\theta}_d^A \right) \text{diag}\left(\ddot{\boldsymbol{\lambda}_d}\right)$. We observe that $\mathbf{Z}_d \mathbf{Z}_d^\top = \widehat{\mathbf{C}}_d$ acts as an empirical covariance matrix for the sinusoidal features $\Omega_\mathcal{Q}^d$ and $\Omega_\mathcal{K}^d$. Since $\mathbf{Z}_d$ has zero mean and unit variance, as $R \to \infty$, $\widehat{\mathbf{C}}_d$ approaches the theoretical covariance matrix $\mathbf{C}_d = \mathbf{I}_{2K}$.
In the ideal case of $\mathbf{C}_d$, Equation \ref{eq:sff_mn} simplifies to $\mathbf{P}_d[m, n] \approx \Omega_\mathcal{Q}^d [m, :] \Omega_\mathcal{K}^{d^\top} [:, n]$, giving:
\begin{equation} \label{eq:ideal_C}
    \mathbf{P}_d[m, n] \approx  \frac{1}{N_f}  \sum_{\omega = 1}^{N_f} \Lambda_\omega \cos \big( f_{\omega} ( \mathcal{P}_Q[m] - \mathcal{P}_K[n] ) + \Theta_\omega \big)
\end{equation}
where $\Lambda_\omega$ is the gain contributed by the matrices $\text{diag}\left(\ddot{\boldsymbol{\lambda}_d}\right)$ and $\Theta_\omega$ is the phase-shift contributed by $\boldsymbol{\theta}^Q_d$ and $\boldsymbol{\theta}^K_d$.

This representation has been studied in previous work, where it is called \textit{Random Fourier Features} (RFF) \cite{rahimi_random_2007, sutherland_error_2015}.

\subsection{F-StrIPE}

We can redesign the positional feature matrices to be:
\begin{equation} \label{eq:rff}
    \mathbf{P}^{Q/K}_d = \boldsymbol{\Omega}\left(\mathcal{P}_{Q/K}, \boldsymbol{f}_d, \boldsymbol{\theta}_d^{Q/K}\right) \text{diag}\left(\ddot{\boldsymbol{\lambda}_d}\right) / \sqrt{N_f}
\end{equation}
where the sinusoidal feature matrix $\boldsymbol{\Omega}$ is given by:
\begin{equation} \label{eq:sff:sinusoidal_features}
    [\boldsymbol{\Omega}(\mathcal{P}, \boldsymbol{f}, \boldsymbol{\theta})]_{i j}= \begin{cases}\cos \left(2 \pi \mathbf{f}[\omega, :]^\top p_i+\boldsymbol{\theta}[\omega]\right) & \text { if } j = 2\omega \\ \sin \left(2 \pi \mathbf{f}[\omega, :]^\top p_i+\boldsymbol{\theta}[\omega] \right) & \text { else }\end{cases}
\end{equation}
Here, unlike (\ref{eq:sff:sine_features}) where $\mathbf{f}[\omega]$ was a single frequency, $\mathbf{f}[\omega, :]$ is a vector of frequencies. Each frequency $\mathbf{f}[\omega, \ell]$ in this vector acts on the $\ell^{\text{th}}$ structural label at timestep $i$, where we can use the vectorial formulation of structure-aware positional indices $p_i = \mathbf{s}(i)$.

With this, we can now formulate F-StrIPE by modifying (\ref{eq:spe:ohyeah}) to use $\mathbf{P}^{Q/K}_d$ in place of $\thicktilde{\mathbf{P}}^{Q/K}_d$, giving us $\mathbf{Q}^{\text{RFF}}/\mathbf{K}^{\text{RFF}}$ in place of $\mathbf{Q}^{\text{SFF}}/\mathbf{K}^{\text{SFF}}$. In the second row of Figure \ref{fig:visualize_matrices}, similar to SFF, we show the different components of RFF in the case where we assume gains to be 1 and phase shifts to be 0. RFF can be understood as the ideal case of SFF where $R \to \infty$. Seen in this way, RFF can give us a noiseless estimate of $\mathbf{P}_d$ with direct access to the theoretical covariance matrix $\mathbf{C}_d$.

In addition, if we pair $\mathbf{Q}^{\text{SFF}}/\mathbf{K}^{\text{SFF}}$ with the sinusoidal features given in Equation \ref{eq:sff:sinusoidal_features}, in place of those given in Equation \ref{eq:sff:sine_features}, we obtain a richer version of SPE which accepts multi-dimensional structural information instead of time indices. To distinguish it from SPE, we name this variant F-StrIPE:SFF.

\subsection{Assessing with music generation}

\subsubsection{Dataset and Input Representation} \label{sssection:data_input}
We use the Chinese POP909 dataset~\cite{wang_pop909_2020} and three levels of structural labels with different resolutions~\cite{dai_automatic_2020}: melodic pitch ($16^{th}$-note), chord (quarter-note) and phrase (bar). Each MIDI file in this dataset consists of three tracks: melody, bridge (second melody) and piano (accompaniment). 
We use the POP909 alignment dataset~\cite{agarwal_structure_2024} to correctly match the structural labels with the input. We convert the MIDI files to binary pianorolls $\mathbf{X} \in \mathbb{B}^{(n_\text{tracks} \times 128) \times n_\text{time}}, \mathbb{B} = \{0, 1\}$, where $n_\text{tracks}$ is the number of tracks and $n_\text{time}$ is the number of timesteps in the pianoroll.

\subsubsection{Task Setup}
We use a symbolic music generation task, namely, melody harmonization, to test the efficacy of our method. Given the pianoroll for the melody and bridge tracks $\left[ \mathbf{x}_n \in \mathbb{B}^{(n_\text{tracks} - 1) \times 128} \right]$, the model must predict all tracks $\left[ \mathbf{y}_n \in \mathbb{B}^{n_\text{tracks} \times 128} \right]$. We expect the model to predict the complete accompaniment track for all timesteps at once, without conditioning later predictions on earlier predictions. 
% We use three settings: (16, 16), (16, 64) and (64, 64), where the first number is the sequence length (in bars of music) used for training and the second number is that used for testing.
We use two settings: (16, 16) and (16, 64), where the first number is the sequence length (in bars of music) used for training and the second number is that used for testing.

\subsubsection{Model and Training}
We use a 2-layer causal encoder Transformer with 4 heads and 512 model dimension. Training for 15 epochs with a batch size of 8, we use gradient clipping and curriculum learning~\cite{bengio_curriculum_2009}. We use two learning rate schedulers: a linear warmup and an epoch-wise decay.
We do a grid-search for two hyperparameters: learning rate (choices: $\{ 1, 5, 10 \} \times 0.0001$) and post-processing binarization strategy~\cite{agarwal_structure_2024} (choices: thresholding, thresholding with merge). The thresholding strategy binarizes based on a fixed threshold and the thresholding with merge strategy allows us to additionally fill in the gap between two binary notes if the gap is less than a minimum merge distance.

\subsubsection{Baselines and Our Methods} \label{sssection:baselines}
We consider three types of baselines: (i) Transformers without PE (NoPE), (ii) Transformers with efficient, approximate atttention but no structural information in PE (SPE~\cite{liutkus_relative_2021}), and (iii) Transformers with structural information in PE but using inefficient, exact attention (S S-RPE~\cite{agarwal_structure_2024}).
From our methods, we use F-StrIPE with the three structural levels described in Section \ref{sssection:data_input}. We also assess the influence of different random features with F-StrIPE:SFF using all structural levels. 
We perform ablations on F-StrIPE by selecting one level at a time during training. Finally, we use the best-performing structural level from the F-StrIPE ablations to additionally do an ablation study with F-StrIPE:SFF.

\subsubsection{Evaluation}
To compare our predictions with the targets, we choose a collection of musically-motivated metrics from the literature guided by four criteria. To assess large- and small-scale structural properties, we use Self-Similarity Matrix Distance (SSMD)~\cite{wu_musemorphose_2021}, where we compute the mean absolute difference between self-similarity matrices obtained from the pairwise cosine similarity of the chromas of the target music and generated music. For rhythmic and melodic consistency, we use Grooving pattern Similarity (GS)~\cite{wu_jazz_2020} and Chroma Similarity (CS)~\cite{wu_musemorphose_2021}, respectively. GS is the overlap between the note onset histograms of the target and prediction, whereas CS is the average cosine similarity between the chroma onset vectors of the target and prediction. To gauge polyphonicity, we use Note Density Distance (NDD)~\cite{agarwal_structure_2024, haki_real_2022}, which is the mean absolute difference in note density between the target and prediction. For a more detailed description of the metrics, we refer readers to previous work~\cite{agarwal_structure_2024}.


==> sections/results_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[t]
%\sisetup{round-mode=places}
\centering
\resizebox{2.1\columnwidth}{!}{%
\begin{tabular}{lcccccccccccc}
%{S[round-precision=1]}
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Method}}} & \multicolumn{4}{c|}{\textbf{Train = 16 bars; Test = 16 bars}} & \multicolumn{4}{c|}{\textbf{Train = 16 bars; Test = 64 bars}} & \multicolumn{4}{c}{\textbf{Train = 64 bars; Test = 64 bars}} \\
\multicolumn{1}{c|}{} & \textbf{CS} & \textbf{SSMD} & \textbf{GS} & \multicolumn{1}{c|}{\textbf{NDD}} & \textbf{CS} & \textbf{SSMD} & \textbf{GS} & \multicolumn{1}{c|}{\textbf{NDD}} & \textbf{CS} & \textbf{SSMD} & \textbf{GS} & \textbf{NDD} \\
\multicolumn{1}{c|}{} & $\uparrow$ & $\downarrow$ & $\uparrow$ & \multicolumn{1}{c|}{$\downarrow$} & $\uparrow$ & $\downarrow$ & $\uparrow$ & \multicolumn{1}{c|}{$\downarrow$} & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ \\ \hline \hline
\multicolumn{1}{l|}{\textbf{NoPE}} & \phantom{0}2.7 $\pm$ 0.2 & 29.3 $\pm$ 0.0 & \phantom{0}7.8 $\pm$ 0.1 & \multicolumn{1}{c|}{103.2 $\pm$ 0.0} & \phantom{0}2.7 $\pm$ 0.2 & 27.6 $\pm$ 0.0 & \phantom{0}9.8 $\pm$ 0.6 & \multicolumn{1}{c|}{102.5 $\pm$ 0.1} & \phantom{0}2.7 $\pm$ 1.9 & 27.6 $\pm$ 0.0 & \phantom{0}9.5 $\pm$ 6.2 & 102.5 $\pm$ 0.6 \\
\multicolumn{1}{l|}{\textbf{S S-RPE}~\cite{agarwal_structure_2024}} & 14.5 $\pm$ 0.7 & 28.9 $\pm$ 0.1 & 21.6 $\pm$ 0.9 & \multicolumn{1}{c|}{\phantom{0}98.9 $\pm$ 0.4} & $\diagdown$ & $\diagdown$ & $\diagdown$ & \multicolumn{1}{c|}{$\diagdown$} & $\diagdown$ & $\diagdown$ & $\diagdown$ & $\diagdown$ \\
\multicolumn{1}{l|}{\textbf{SPE}~\cite{liutkus_relative_2021}} & \phantom{0}1.1 $\pm$ 0.0 & 29.3 $\pm$ 0.0 & \phantom{0}6.0 $\pm$ 0.0 & \multicolumn{1}{c|}{103.8 $\pm$ 0.0} & \phantom{0}6.7 $\pm$ 0.3 & 27.6 $\pm$ 0.0 & 20.3 $\pm$ 0.7 & \multicolumn{1}{c|}{101.7 $\pm$ 0.1} & \phantom{0}3.2 $\pm$ 0.1 & 27.6 $\pm$ 0.0 & 11.9 $\pm$ 0.5 & 102.3 $\pm$ 0.1 \\ \hline
\multicolumn{1}{l|}{\textbf{F-StrIPE:SFF}} & \phantom{0}2.8 $\pm$ 3.0 & 29.3 $\pm$ 0.0 & \phantom{0}8.2 $\pm$ 3.5 & \multicolumn{1}{c|}{103.4 $\pm$ 0.7} & \phantom{0}6.5 $\pm$ 0.3 & 27.6 $\pm$ 0.0 & 20.5 $\pm$ 0.7 & \multicolumn{1}{c|}{101.7 $\pm$ 0.1} & \phantom{0}5.0 $\pm$ 0.5 & 27.6 $\pm$ 0.0 & 16.6 $\pm$ 1.6 & 102.1 $\pm$ 0.1 \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:SFF:C}} & \phantom{0}4.7 $\pm$ 3.9 & 29.3 $\pm$ 0.1 & 10.2 $\pm$ 4.6 & \multicolumn{1}{c|}{102.5 $\pm$ 1.3} & 10.4 $\pm$ 1.0 & 27.4 $\pm$ 0.1 & 29.8 $\pm$ 1.9 & \multicolumn{1}{c|}{\phantom{0}99.9 $\pm$ 0.5} & \phantom{0}4.7 $\pm$ 0.5 & 27.5 $\pm$ 0.0 & 15.9 $\pm$ 0.8 & 101.6 $\pm$ 0.1 \\ \hline
\multicolumn{1}{l|}{\textbf{F-StrIPE}}  & 11.8 $\pm$ 1.2 & 29.2 $\pm$ 0.0 & 18.6 $\pm$ 1.4 & \multicolumn{1}{c|}{100.8 $\pm$ 0.4} & \phantom{0}9.1 $\pm$ 1.2 & 27.5 $\pm$ 0.0 & 27.4 $\pm$ 2.9 & \multicolumn{1}{c|}{100.8 $\pm$ 0.2} & \phantom{0}5.3 $\pm$ 0.5 & 27.6 $\pm$ 0.0 & 17.1 $\pm$ 1.5 & 102.1 $\pm$ 0.1 \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:M}} & \phantom{0}1.9 $\pm$ 0.1 & 29.3 $\pm$ 0.0 & \phantom{0}7.1 $\pm$ 0.1 & \multicolumn{1}{c|}{103.5 $\pm$ 0.0} & \phantom{0}2.2 $\pm$ 0.1 & 27.6 $\pm$ 0.0 & \phantom{0}8.4 $\pm$ 0.5 & \multicolumn{1}{c|}{102.7 $\pm$ 0.0} & \phantom{0}0.0 $\pm$ 0.0 & 27.6 $\pm$ 0.0 & \phantom{0}0.8 $\pm$ 0.0 & 103.4 $\pm$ 0.0 \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:C}} & \textbf{16.6 $\pm$ 1.5} & \textbf{28.7 $\pm$ 0.1} & \textbf{23.2 $\pm$ 2.7} & \multicolumn{1}{c|}{\textbf{\phantom{0}97.1 $\pm$ 0.4}} & \textbf{13.3 $\pm$ 1.1} & \textbf{27.2 $\pm$ 0.1} & \textbf{37.8 $\pm$ 2.7} & \multicolumn{1}{c|}{\textbf{\phantom{0}97.1 $\pm$ 0.3}} & \textbf{\phantom{0}7.2 $\pm$ 0.4} & \textbf{27.4 $\pm$ 0.1} & \textbf{23.2 $\pm$ 1.6} & \textbf{100.3 $\pm$ 0.2} \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:P}} & \phantom{0}2.1 $\pm$ 0.1 & 29.3 $\pm$ 0.0 & \phantom{0}7.2 $\pm$ 0.1 & \multicolumn{1}{c|}{103.4 $\pm$ 0.0} & \phantom{0}2.3 $\pm$ 0.1 & 27.6 $\pm$ 0.0 & \phantom{0}9.1 $\pm$ 0.3 & \multicolumn{1}{c|}{102.6 $\pm$ 0.0} & \phantom{0}0.0 $\pm$ 0.0 & 27.6 $\pm$ 0.0 & \phantom{0}0.8 $\pm$ 0.0 & 103.4 $\pm$ 0.0 \\ \hline
\end{tabular}
}
\caption{Performance on melody harmonization. F-StrIPE:(M/C/P) are the ablations on F-StrIPE, described in Section \ref{sssection:baselines}, that apply RFF on only one structural level at a time - melodic pitch/chord/phrase. F-StrIPE:SFF:C applies SFF on chords, which is the best performing ablation setting with RFF.}
\label{tab:results}
\end{table*}

==> sections/results_table_2decimals.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\resizebox{2.05\columnwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Method}}} & \multicolumn{4}{c|}{\textbf{Train = 16 bars; Test = 16 bars}} & \multicolumn{4}{c}{\textbf{Train = 16 bars; Test = 64 bars}} \\
\multicolumn{1}{c|}{} & \textbf{CS} & \textbf{SSMD} & \textbf{GS} & \multicolumn{1}{c|}{\textbf{NDD}} & \textbf{CS} & \textbf{SSMD} & \textbf{GS} & \multicolumn{1}{c}{\textbf{NDD}}\\
\multicolumn{1}{c|}{} & $\uparrow$ & $\downarrow$ & $\uparrow$ & \multicolumn{1}{c|}{$\downarrow$} & $\uparrow$ & $\downarrow$ & $\uparrow$ & \multicolumn{1}{c}{$\downarrow$} \\ \hline \hline
% \multicolumn{9}{c}{\textbf{Melody Harmonization}} \\ \hline \hline
\multicolumn{1}{l|}{\textbf{NoPE}} & \phantom{0}2.68 $\pm$ 0.16 & 29.31 $\pm$ 0.01 & \phantom{0}7.82 $\pm$ 0.12 & \multicolumn{1}{c|}{103.22 $\pm$ 0.01} & \phantom{0}2.67 $\pm$ 0.18 & 27.60 $\pm$ 0.00 & \phantom{0}9.79 $\pm$ 0.55 & \multicolumn{1}{c}{102.53 $\pm$ 0.05} \\
\multicolumn{1}{l|}{\textbf{S S-RPE}} & 14.52 $\pm$ 0.67 & 28.92 $\pm$ 0.06 & 21.58 $\pm$ 0.86 & \multicolumn{1}{c|}{\phantom{0}98.86 $\pm$ 0.39} & $\diagdown$ & $\diagdown$ & $\diagdown$ & \multicolumn{1}{c}{$\diagdown$} \\
\multicolumn{1}{l|}{\textbf{SPE} \cite{liutkus_relative_2021}} & \phantom{0}1.07 $\pm$ 0.04 & 29.33 $\pm$ 0.00 & \phantom{0}6.02 $\pm$ 0.02 & \multicolumn{1}{c|}{103.81 $\pm$ 0.02} & \phantom{0}6.71 $\pm$ 0.28 & 27.59 $\pm$ 0.00 & 20.27 $\pm$ 0.65 & \multicolumn{1}{c}{101.69 $\pm$ 0.06}\\ \hline
\multicolumn{1}{l|}{\textbf{F-StrIPE}}  & 11.84 $\pm$ 1.24 & 29.18 $\pm$ 0.03 & 18.62 $\pm$ 1.44 & \multicolumn{1}{c|}{100.78 $\pm$ 0.43} & \phantom{0}9.13 $\pm$ 1.19 & 27.53 $\pm$ 0.00 & 27.42 $\pm$ 2.90 & \multicolumn{1}{c}{100.79 $\pm$ 0.21} \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:M}} & \phantom{00}1.9 $\pm$ 0.09 & 29.31 $\pm$ 0.01 & \phantom{0}7.07 $\pm$ 0.13 & \multicolumn{1}{c|}{103.48 $\pm$ 0.03} & \phantom{0}2.22 $\pm$ 0.13 & 27.60 $\pm$ 0.00 & \phantom{0}8.43 $\pm$ 0.50 & \multicolumn{1}{c}{102.69 $\pm$ 0.01} \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:C}} & 16.61 $\pm$ 1.52 & 28.71 $\pm$ 0.07 & 23.19 $\pm$ 2.71 & \multicolumn{1}{c|}{\phantom{0}97.14 $\pm$ 0.37} & 13.29 $\pm$ 1.08 & 27.15 $\pm$ 0.10 & 37.80 $\pm$ 2.74 & \multicolumn{1}{c}{\phantom{0}97.08 $\pm$ 0.34} \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:P}} & \phantom{0}2.07 $\pm$ 0.10 & 29.31 $\pm$ 0.01 & \phantom{0}7.23 $\pm$ 0.14 & \multicolumn{1}{c|}{103.43 $\pm$ 0.02} & \phantom{0}2.31 $\pm$ 0.09 & 27.60 $\pm$ 0.00 & \phantom{0}9.11 $\pm$ 0.27 & \multicolumn{1}{c}{102.64 $\pm$ 0.02} \\ \hline
\multicolumn{1}{l|}{\textbf{F-StrIPE:SFF}} & \phantom{0}2.75 $\pm$ 3.01 & 29.32 $\pm$ 0.03 & \phantom{0}8.15 $\pm$ 3.46 & \multicolumn{1}{c|}{103.43 $\pm$ 0.74} & \phantom{0}6.49 $\pm$ 0.34 & 27.58 $\pm$ 0.00 & 20.50 $\pm$ 0.65 & \multicolumn{1}{c}{101.69 $\pm$ 0.10} \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:SFF:C}} & \phantom{0}4.72 $\pm$ 3.86 & 29.25 $\pm$ 0.07 & 10.22 $\pm$ 4.63 & \multicolumn{1}{c|}{102.54 $\pm$ 1.26} & 10.35 $\pm$ 0.95 & 27.44 $\pm$ 0.05 & 29.81 $\pm$ 1.94 & \multicolumn{1}{c}{\phantom{0}99.88 $\pm$ 0.50} \\ \hline
\end{tabular}
}
\caption{Performance on melody harmonization. F-StrIPE:(M/C/P) are the ablations on F-StrIPE, described in Section \ref{sssection:baselines}, that apply RFF on only one structural level at a time - melodic pitch/chord/phrase. F-StrIPE:SFF:C applies SFF on chords, which is the best performing ablation setting with RFF.}
\label{tab:results_unrounded}
\end{table*}

==> sections/results_table_std_rounded.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\resizebox{2.05\columnwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Method}}} & \multicolumn{4}{c|}{\textbf{Train = 16 bars; Test = 16 bars}} & \multicolumn{4}{c}{\textbf{Train = 16 bars; Test = 64 bars}} \\
\multicolumn{1}{c|}{} & \textbf{CS} & \textbf{SSMD} & \textbf{GS} & \multicolumn{1}{c|}{\textbf{NDD}} & \textbf{CS} & \textbf{SSMD} & \textbf{GS} & \multicolumn{1}{c}{\textbf{NDD}}\\
\multicolumn{1}{c|}{} & $\uparrow$ & $\downarrow$ & $\uparrow$ & \multicolumn{1}{c|}{$\downarrow$} & $\uparrow$ & $\downarrow$ & $\uparrow$ & \multicolumn{1}{c}{$\downarrow$} \\ \hline \hline
% \multicolumn{9}{c}{\textbf{Melody Harmonization}} \\ \hline \hline
\multicolumn{1}{l|}{\textbf{NoPE}} & \phantom{0}2.68 $\pm$ 0.2\phantom{*} & 29.31 $\pm$ 0.0* & \phantom{0}7.82 $\pm$ 0.1\phantom{*} & \multicolumn{1}{c|}{103.22 $\pm$ 0.0*} & \phantom{0}2.67 $\pm$ 0.2 & 27.60 $\pm$ 0.0* & \phantom{0}9.79 $\pm$ 0.6 & \multicolumn{1}{c}{102.53 $\pm$ 0.1\phantom{*}} \\
\multicolumn{1}{l|}{\textbf{S S-RPE}} & 14.52 $\pm$ 0.7\phantom{*} & 28.92 $\pm$ 0.1\phantom{*} & 21.58 $\pm$ 0.9\phantom{*} & \multicolumn{1}{c|}{\phantom{0}98.86 $\pm$ 0.4\phantom{*}} & $\diagdown$ & $\diagdown$ & $\diagdown$ & \multicolumn{1}{c}{$\diagdown$} \\
\multicolumn{1}{l|}{\textbf{SPE} \cite{liutkus_relative_2021}} & \phantom{0}1.07 $\pm$ 0.0* & 29.33 $\pm$ 0.0* & \phantom{0}6.02 $\pm$ 0.0* & \multicolumn{1}{c|}{103.81 $\pm$ 0.0*} & \phantom{0}6.71 $\pm$ 0.3 & 27.59 $\pm$ 0.0* & 20.27 $\pm$ 0.7 & \multicolumn{1}{c}{101.69 $\pm$ 0.1\phantom{*}}\\ \hline
\multicolumn{1}{l|}{\textbf{F-StrIPE}}  & 11.84 $\pm$ 1.2\phantom{*} & 29.18 $\pm$ 0.0* & 18.62 $\pm$ 1.4\phantom{*} & \multicolumn{1}{c|}{100.78 $\pm$ 0.4\phantom{*}} & \phantom{0}9.13 $\pm$ 1.2 & 27.53 $\pm$ 0.0* & 27.42 $\pm$ 2.9 & \multicolumn{1}{c}{100.79 $\pm$ 0.2\phantom{*}} \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:M}} & \phantom{00}1.9 $\pm$ 0.1\phantom{*} & 29.31 $\pm$ 0.0* & \phantom{0}7.07 $\pm$ 0.1\phantom{*} & \multicolumn{1}{c|}{103.48 $\pm$ 0.0*} & \phantom{0}2.22 $\pm$ 0.1 & 27.60 $\pm$ 0.0* & \phantom{0}8.43 $\pm$ 0.5 & \multicolumn{1}{c}{102.69 $\pm$ 0.0*} \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:C}} & \textbf{16.61 $\pm$ 1.5\phantom{*}} & \textbf{28.71 $\pm$ 0.1\phantom{*}} & \textbf{23.19 $\pm$ 2.7\phantom{*}} & \multicolumn{1}{c|}{\textbf{\phantom{0}97.14 $\pm$ 0.4\phantom{*}}} & \textbf{13.29 $\pm$ 1.1} & \textbf{27.15 $\pm$ 0.1\phantom{*}} & \textbf{37.80 $\pm$ 2.7} & \multicolumn{1}{c}{\textbf{\phantom{0}97.08 $\pm$ 0.3\phantom{*}}} \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:P}} & \phantom{0}2.07 $\pm$ 0.1\phantom{*} & 29.31 $\pm$ 0.0* & \phantom{0}7.23 $\pm$ 0.1\phantom{*} & \multicolumn{1}{c|}{103.43 $\pm$ 0.0*} & \phantom{0}2.31 $\pm$ 0.1 & 27.60 $\pm$ 0.0* & \phantom{0}9.11 $\pm$ 0.3 & \multicolumn{1}{c}{102.64 $\pm$ 0.0*} \\ \hline
\multicolumn{1}{l|}{\textbf{F-StrIPE:SFF}} & \phantom{0}2.75 $\pm$ 3.0\phantom{*} & 29.32 $\pm$ 0.0* & \phantom{0}8.15 $\pm$ 3.5\phantom{*} & \multicolumn{1}{c|}{103.43 $\pm$ 0.7\phantom{*}} & \phantom{0}6.49 $\pm$ 0.3 & 27.58 $\pm$ 0.0* & 20.50 $\pm$ 0.7 & \multicolumn{1}{c}{101.69 $\pm$ 0.1\phantom{*}} \\
\multicolumn{1}{l|}{\textbf{F-StrIPE:SFF:C}} & \phantom{0}4.72 $\pm$ 3.9\phantom{*} & 29.25 $\pm$ 0.1\phantom{*} & 10.22 $\pm$ 4.6\phantom{*} & \multicolumn{1}{c|}{102.54 $\pm$ 1.3\phantom{*}} & 10.35 $\pm$ 1.0 & 27.44 $\pm$ 0.1\phantom{*} & 29.81 $\pm$ 1.9 & \multicolumn{1}{c}{\phantom{0}99.88 $\pm$ 0.5\phantom{*}} \\ \hline
\end{tabular}
}
\caption{Performance on melody harmonization. F-StrIPE:(M/C/P) are the ablations on F-StrIPE, described in Section \ref{sssection:baselines}, that apply RFF on only one structural level at a time - melodic pitch/chord/phrase. F-StrIPE:SFF:C applies SFF on chords, which is the best performing ablation setting with RFF. `0.0*' refers to standard deviations that are lower than 0.05. `$\diagdown$' refers to simulations where the given inference setting could not be accessed due to the heavy computational demands of the method.}
\label{tab:results_unrounded}
\end{table*}
